Design and Control of a VTOL Aerial Vehicle Tilting its Rotors Only with Rotor Thrusts and a Passive Joint

This paper presents a novel VTOL UAV that owns a link connecting four rotors and a fuselage by a passive joint, allowing the control of the rotor's tilting angle by adjusting the rotors' thrust. This unique structure contributes to eliminating additional actuators, such as servo motors, to control the tilting angles of rotors, resulting in the UAV's weight lighter and simpler structure. We first derive the dynamical model of the newly designed UAV and analyze its controllability. Then, we design the controller that leverages the tiltable link with four rotors to accelerate the UAV while suppressing a deviation of the UAV's angle of attack from the desired value to restrain the change of the aerodynamic force. Finally, the validity of the proposed control strategy is evaluated in simulation study.

==> text/2-model.tex <==
% \documentclass[ieeeconf]{subfiles}
% \begin{document}
%%============================================================================%%
\section{MODELING}

\begin{figure}[t]
    % \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{"figure/modeling/topview.eps"}
        \caption{topview}
        \label{fig:topview}
    % \end{minipage}\hspace{2em}
\end{figure}
\begin{figure}[t]
        % \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{"figure/modeling/sideview.eps"}
        \caption{sideview}
        \label{fig:sideview}
    % \end{minipage}   
\end{figure}
\begin{figure*}[t]
        % \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{"figure/modeling/transition.eps"}
        \caption{transition}
        \label{fig:transition}
    % \end{minipage}   
\end{figure*}

This section introduces the overview of the proposed vehicle, the formulation of transforming rotor thrusts into body forces and torques, and the equation of motion for rigid body dynamics.

\subsection{Overview of the Vehicle}
The kinematic parameters of the aerial vehicle, including its position and attitude, are expressed within several coordinate frame systems.
We define the ground-fixed inertial frame as the NED (North-East-Down) frame, while the body-fixed frame follows a right-hand coordinate system, with the $x$-axis oriented forward, the $y$-axis oriented to the right, and the positive $z$-axis pointing downward. The stability frame is obtained by rotating the body frame around the $y$-axis to make the velocity in the $z$-direction zero. This rotational angle is referred to as the angle of attack, denoted as character $\alpha$.
A left-side superscript means coordinate frame, where $b$ means the body frame, $i$ means the inertial frame, and $s$ means the stability frame.

The overview of the aerial vehicle is shown in Figs.~\ref{fig:topview} and \ref{fig:sideview}.
The vehicle comprises a fuselage, six rotors, and a single link. This link is connected to the fuselage and can freely rotate around the y-axis of the body frame. It is named the quadlink, consisting of the first to fourth rotors, as depicted in Fig.~\ref{fig:topview}. The remaining two rotors, the fifth and sixth, are fixed directly to the fuselage.

The tilt angle of the quadlink with respect to the body frame is denoted as $\chi$. Its value becomes zero when the rotors are directed upward and reaches $-\pi/2$ when they are oriented fully forward. The control of $\chi$ is achieved through the manipulation of the thrust generated by the rotors within the quadlink.

This vehicle distinguishes itself from conventional tiltrotor vehicles due to its unique tilt mechanism, which relies on a passive joint controlled solely by rotor thrusts. Notably, this vehicle is controlled without any control surfaces, such as a rudder, aileron, or elevator. This means that we eliminate the requirement for additional actuators, resulting in a reduction in overall weight.
% この機体は，conventionalなtiltrotorと違い，ロータ傾斜機構にpassive jointを採用してその傾斜角度の制御をロータの推力で行うところがuniqueである．さらに本論文ではエルロンやラダーなどのcontrol surfaceを導入せずに制御することに成功している．
% これらから，本機体は追加のアクチュエータなどが必要なく，重量増加を抑えることができる．

One of the most challenging aspects of VTOL control lies in the transition from hovering mode to cruise flight mode. To address this challenge, we employ a four-phase transition strategy as shown in Fig.~\ref{fig:transition} and utilize gain-scheduling techniques.
The four transition phases are as follows:
\begin{enumerate}
    \item Hovering Phase: During this phase, the vehicle takes off vertically and remains in a static hover position in mid-air. The tilt angle $\chi$ is controlled to maintain a zero value.
    \item Ready Phase: In the Ready Phase, the vehicle smoothly transitions to the planned initial $\alpha$ and $\chi$ angles, preparing for the Acceleration Phase while still in hover mode.
    \item Acceleration Phase: The vehicle accelerates forward during this phase until it reaches the target forward velocity. Nonlinear aerodynamic effects change in response to the evolving vehicle states during the transition, making it challenging to control the vehicle with a single static controller. Therefore, we implement gain scheduling to adapt to these dynamic variations.
    \item Cruise Phase: In the Cruise Phase, the vehicle maintains stable flight while keeping the target velocity constant.
\end{enumerate}
% At first, the vehicle hovers at one point, then second, it transitions into the initial pose of third phase acceleration, finally settling on the cruise with a certain velocity. 
Detailed controllers are described in Section 4.
% この機体は，最終的にFig.~\ref{fig:transition}に示すように複数のフェーズを経て制御される．はじめに空中でホバリングしてから，加速の準備状態へと移行し，加速した後一定速度で飛行するcruise状態で落ち着く．それぞれのフェーズの詳細は4章のCONTROLLERで詳細に述べている．なお，これらのTransitionはすべてロータの推力のみで制御される，

% 本研究で扱う機体の概要をfig.\ref{fig:topview}, \ref{fig:sideview}に示す．
% 機体軸系には，機体の前方に$x$軸を，右側に$y$軸を，下方向に$z$をとる右手座標系を用いる．
% また，機体軸系を$y$軸回りに回転させ$z$軸方向の速度をゼロにした座標系を安定軸系という．
% このときの機体軸系と安定軸系の間の角度を迎角といい，$\alpha$で表す．

% 機体はロータ6枚で構成され，ロータのインデックスは図に示すとおりである．
% また，fig.\ref{fig:topview}の$l_{\ast}$はそれぞれ長さを示しており，飛行中に変わらない一定の値である．
% 機体前方の4枚はy軸方向の一軸周りに自由に回転するジョイントで接続されたリンク上に配置され，これをクアッドリンクと呼ぶ．
% クアッドリンクの機体に対する傾き角はロータの回転数を調整することで制御できる．
% この傾斜角を$\chi$で表す．なおロータの推力が機体上向き方向に向いているときを$\chi=0$とし，
% 完全に前方を向いた時に$\chi=-\pi/2$を取る．

% 翼の揚力と抗力が作用する中心点は機体重心と一致しており，空力による重心周りのモーメントは無視することができるとする．

\subsection{Transformation of the Rotor Thrusts(座標追加)}
ロータ推力は$f_i$，反トルク係数は$\kappa_i=\pm \kappa$であり，符号はCWのとき正，CCWのとき負である．このときロータの推力は
\begin{align}
    \bm f_i = \begin{bmatrix}
        0 & 0 & f_i & 0 & 0 & \pm\kappa_i f_i
    \end{bmatrix}
\end{align}
となる．リンク座標に変換すると．
\begin{align}
    \begin{bmatrix}
    \bm  f_\text{link} \\ \bm \tau_\text{link}
    \end{bmatrix} =
    \sum^4_{i=1} (\bm p_{link2i}\times \bm f_i + \kappa_i \bm f_i)
\end{align}
これを機体座標に変換すると．
\begin{align}
    \begin{bmatrix}
    \bm  f_\text{link} \\ \bm \tau_\text{link}
    \end{bmatrix} = \begin{bmatrix}
        \bm R_y(\chi) & \bm O_3 \\
        \hat{bm p}_{body2link}\bm R_y(\chi) & \bm R_y(\chi)
    \end{bmatrix}
    \begin{bmatrix}
    \bm  f_\text{link} \\ \bm \tau_\text{link}
    \end{bmatrix}
    + \sum^6_{i=5} (\bm p_{body2i}\times \bm f_i + \kappa_i \bm f_i)
\end{align}
となる．

\subsection{Transformation of the Rotor Thrusts}
The i-th rotor generates an upward thrust denoted as $\bm f_i = [0~0~f_i]^\top$ and an opposing proportional counter-torque represented as $\bm \tau_i = \kappa_i \bm f_i$, where $\kappa$ is the constant of proportionality. The sign of $\kappa$ is positive when the rotor rotates clockwise and negative when it rotates counterclockwise. Neglecting any drag forces between the fuselage and the quadlink, the torque around the joint axis is solely responsible for rotating the quadlink.
Let $\bm p_i$ be the vector from the gravity center of the vehicle to the point that loaded force as shown in Table~\ref{tab:pi} with the symbols in Fig.~\ref{fig:topview}.
\begin{table}[h]
    \caption{The definition of $\bm p_i$}
    \label{tab:pi}
    \begin{center}
    \begin{tabular}{|c||c|}
        \hline
        $\bm p_1,~\bm p_2$ & $[l_f~l_{fw}]^\top$\\
        $\bm p_3,~\bm p_4$ & $[l_f~-l_{fw}]^\top$\\
        $\bm p_5$ & $[-l_b~-l_{bw}]^\top$\\
        $\bm p_6$ & $[-l_b~l_{bw}]^\top$\\
        \hline
    \end{tabular}
    \end{center}
\end{table}
Consequently, the force and torque acting on the fuselage can be expressed through coordinate transformation and the summation of rotor thrusts as follows.
\begin{align}
    ^{b} \bm f_\text{rot} =& \bm R_y(\chi)\sum^4_{i=1} \bm f_i + \sum^6_{i=5} \bm f_i, \label{eq:Frotor} \\
    ^{b} \bm \tau_\text{rot} =& \bm R_y(\chi) 
                            \begin{bmatrix}
                                1 & 0 & 0 \\
                                0 & 0 & 0 \\
                                0 & 0 & 1
                            \end{bmatrix} % \mathrm{diag}(1,~0,~1)
                            \sum^4_{i=1} \left( \bm p_i\times \bm f_i +\kappa_i \bm f_i \right)\notag \\
                            & + \sum^6_{i=5} \left(\bm p_i\times \bm f_i +\kappa_i \bm f_i \right), \label{eq:Mrotor}
\end{align}
The torque applied to the quadlink can be formulated as 
\begin{align}
    \tau_\chi = \begin{bmatrix}
                    0 & 1 & 0
                \end{bmatrix}
                \sum^4_{i=1} \left( \bm p_i\times f_i \bm e_3 +\kappa_i f_i \bm e_3 \right).\label{eq:tau_chi}
\end{align}
Considering that the rotor thrust vector is defined as $\bm f_\text{rot} = [f_1 \cdots f_6]^\top$, Eq.~\eqref{eq:Frotor}, \eqref{eq:Mrotor}, and \eqref{eq:tau_chi} can be expressed in matrix form as follows.
\begin{align}
    ^{b} \bm f_\text{rot} =& 
    \begin{bmatrix}
        - S_\chi & - S_\chi & - S_\chi & - S_\chi & 0 & 0 \\
        0 & 0 & 0 & 0 & 0 & 0 \\
        - C_\chi & - C_\chi & - C_\chi & - C_\chi & -1 & -1 \\
    \end{bmatrix} 
    \bm f_\text{rot}, \label{eq:Mf} \\
    ^{b} \bm \tau_\text{rot} =& 
    \begin{bmatrix}
        -l_{fw} C_\chi-\kappa S_\chi & -l_{fw} C_\chi-\kappa S_\chi & l_{fw} C_\chi+\kappa S_\chi & l_{fw} C_\chi+\kappa S_\chi & -l_{bw} & l_{bw} \\
        l_{f} C_\chi & l_{f} C_\chi & l_{f} C_\chi & l_{f} C_\chi & -l_b & -l_b \\
        l_{fw} S_\chi-\kappa C_\chi & l_{fw} S_\chi-\kappa C_\chi & -l_{fw} S_\chi+\kappa C_\chi & -l_{fw} S_\chi+\kappa C_\chi & \kappa & -\kappa
    \end{bmatrix}
    \bm f_\text{rot}, \label{eq:Mtau} \\
    \tau_\chi =& 
    \begin{bmatrix}
        l_{fh} & -l_{fh} & l_{fh} & -l_{fh} & 0 & 0
    \end{bmatrix}
    \bm f_\text{rot}. \label{eq:Mchi}
\end{align}

% $i$-th rotor generates thrust $\bm f_i = [0~0~f_i]^\top$ upward and proportional counter-torque $\bm \tau_i = \kappa_i \bm f_i$ in the opposite direction, where $\kappa_i$ is a proportional constant. 
% The sign of $\kappa_i$ is positive when the rotor rotates clockwise, while negative when it rotates counter-clockwise. 
% また，クアッドリンクのy軸回りのトルクはジョイントの駆動に使われ，機体には伝達しない．
% このとき，機体に働く推力とモーメントは，ロータ推力の座標返還と合成により次のように表せる．\red{$p$の説明}
% \begin{align}
%     ^{b} \bm f_\text{rot} =& \bm R_y(\chi)\sum^4_{i=1} \bm f_i + \sum^6_{i=5} \bm f_i, \label{eq:Frotor} \\
%     ^{b} \bm \tau_\text{rot} =& \bm R_y(\chi) 
%                             \begin{bmatrix}
%                                 1 & 0 & 0 \\
%                                 0 & 0 & 0 \\
%                                 0 & 0 & 1
%                             \end{bmatrix} % \mathrm{diag}(1,~0,~1)
%                             \sum^4_{i=1} \left( \bm p_i\times \bm f_i +\kappa_i \bm f_i \right)\notag \\
%                             & + \sum^6_{i=5} \left(\bm p_i\times \bm f_i +\kappa_i \bm f_i \right). \label{eq:Mrotor}
% \end{align}
% また，クアッドリンクのジョイント周りのトルクは次式で表される．
% \begin{align}
%     \tau_\chi = \begin{bmatrix}
%                     0 & 1 & 0
%                 \end{bmatrix}
%                 \sum^4_{i=1} \left( \bm p_i\times f_i \bm e_3 +\kappa_i f_i \bm e_3 \right).\label{eq:tau_chi}
% \end{align}
% ロータ推力を並べたベクトルを$\bm f_\text{rot} = [f_1 \cdots f_6]^\top$とすると，
% eq.~\eqref{eq:Frotor}, eq.~\eqref{eq:Mrotor},~\eqref{eq:tau_chi}は$\bm f_\text{rot}$とある行列との積で次のように表せる．
% \begin{align}
%     ^{b} \bm f_\text{rot} =& 
%     \begin{bmatrix}
%         - S_\chi & - S_\chi & - S_\chi & - S_\chi & 0 & 0 \\
%         0 & 0 & 0 & 0 & 0 & 0 \\
%         - C_\chi & - C_\chi & - C_\chi & - C_\chi & -1 & -1 \\
%     \end{bmatrix} 
%     \bm f_\text{rot}, \label{eq:Mf} \\
%     ^{b} \bm \tau_\text{rot} =& 
%     \begin{bmatrix}
%         -l_{fw} C_\chi-\kappa S_\chi & -l_{fw} C_\chi-\kappa S_\chi & l_{fw} C_\chi+\kappa S_\chi & l_{fw} C_\chi+\kappa S_\chi & -l_{bw} & l_{bw} \\
%         l_{f} C_\chi & l_{f} C_\chi & l_{f} C_\chi & l_{f} C_\chi & -l_b & -l_b \\
%         l_{fw} S_\chi-\kappa C_\chi & l_{fw} S_\chi-\kappa C_\chi & -l_{fw} S_\chi+\kappa C_\chi & -l_{fw} S_\chi+\kappa C_\chi & \kappa & -/kappa
%     \end{bmatrix}
%     \bm f_\text{rot}, \label{eq:Mtau} \\
%     \tau_\chi =& 
%     \begin{bmatrix}
%         l_{fh} & -l_{fh} & l_{fh} & -l_{fh} & 0 & 0
%     \end{bmatrix}
%     \bm f_\text{rot}. \label{eq:Mchi}    
% \end{align}

We define new rotor input vectors as $\bm f_\text{r+}= [f_1+f_2,~f_3+f_4,~f_5,~f_6]^\top,\bm f_\text{r-}= [f_1-f_2,~f_3-f_4,~f_5,~f_6]^\top$. Consequently, Eq.~\eqref{eq:Mf}, \eqref{eq:Mtau}, and \eqref{eq:Mchi} can be rewritten as follows. \red{意図を補足}
\begin{align}
    \begin{bmatrix}
        ^{b} \bm f_\text{rot} \\
        ^{b} \bm \tau_\text{rot}
    \end{bmatrix}
    =& \bm M \bm f_\text{r+},\label{eq:M_quad} \\
    \tau_\chi =& 
    \begin{bmatrix}
        l_{fh} & l_{fh} & 0 & 0
    \end{bmatrix}
    \bm f_\text{r-}, \label{eq:Mchi_quad}    
\end{align}
where
\begin{align}
    \bm M = &
    \begin{bmatrix}
        - S_\chi & - S_\chi & 0 & 0 \\
        0 & 0 & 0 & 0 \\
        - C_\chi & - C_\chi & -1 & -1 \\
        -l_{fw} C_\chi-\kappa S_\chi &l_{fw} C_\chi+\kappa S_\chi & -l_{bw} & l_{bw} \\
        l_{f} C_\chi & l_{f} C_\chi & -l_b & -l_b \\
        l_{fw} S_\chi-\kappa C_\chi & -l_{fw} S_\chi+\kappa C_\chi & \kappa & -\kappa
    \end{bmatrix}.\label{eq:M}
\end{align}
Once the desired wrench for the vehicle and the torque for the quadlink are determined, rotor thrusts that generate these desired values can be calculated by inversely transforming Eq. \eqref{eq:M_quad} and \eqref{eq:Mchi_quad}. 
It's important to note that the rank of the matrix in Eq. \eqref{eq:M_quad} is 4, meaning that an inverse transformation may not always exist. However, by adjusting the value of $\chi$, we can derive an equation that allows for a strict inverse transformation.

% ここで新しい入力$\bm f_\text{r+}= [f_1+f_2,~f_3+f_4,~f_5,~f_6]^\top,\bm f_\text{r-}= [f_1-f_2,~f_3-f_4,~f_5,~f_6]^\top$を導入するとeq.~\eqref{eq:Mf}, eq.~\eqref{eq:Mtau}, eq.~\eqref{eq:Mchi}は
% \begin{align}
%     \begin{bmatrix}
%         ^{b} \bm f_\text{rot} \\
%         ^{b} \bm \tau_\text{rot}
%     \end{bmatrix}
%     =& 
%     \begin{bmatrix}
%         - S_\chi & - S_\chi & 0 & 0 \\
%         0 & 0 & 0 & 0 \\
%         - C_\chi & - C_\chi & -1 & -1 \\
%         -l_{fw} C_\chi-\kappa S_\chi &l_{fw} C_\chi+\kappa S_\chi & -l_{bw} & l_{bw} \\
%         l_{f} C_\chi & l_{f} C_\chi & -l_b & -l_b \\
%         l_{fw} S_\chi-\kappa C_\chi & -l_{fw} S_\chi+\kappa C_\chi & \kappa & -\kappa
%     \end{bmatrix}
%     \bm f_\text{r+}, \label{eq:M_quad} \\
%     % ^{b} \bm f_\text{rot} =& 
%     % \begin{bmatrix}
%     %     - S_\chi & - S_\chi & 0 & 0 \\
%     %     0 & 0 & 0 & 0 \\
%     %     - C_\chi & - C_\chi & -1 & -1 \\
%     % \end{bmatrix} 
%     % \bm f_\text{r+}, \label{eq:Mf_quad} \\
%     % ^{b} \bm \tau_\text{rot} =& 
%     % \begin{bmatrix}
%     %     -l_{fw} C_\chi-\kappa S_\chi &l_{fw} C_\chi+\kappa S_\chi & -l_{bw} & l_{bw} \\
%     %     l_{f} C_\chi & l_{f} C_\chi & -l_b & -l_b \\
%     %     l_{fw} S_\chi-\kappa C_\chi & -l_{fw} S_\chi+\kappa C_\chi & \kappa & -\kappa
%     % \end{bmatrix}
%     % \bm f_\text{r+}, \label{eq:Mtau_quad} \\
%     \tau_\chi =& 
%     \begin{bmatrix}
%         l_{fh} & l_{fh} & 0 & 0
%     \end{bmatrix}
%     \bm f_\text{r-}. \label{eq:Mchi_quad}    
% \end{align}
% となる．所望の機体レンチ$[^{b}\bm f_\text{rot}^\top~^{b}\bm\tau_\text{rot}^\top]^\top$を実現する入力$\bm f_\text{r+}$をeq.~\eqref{eq:M_quad}から求め．
% 所望のジョイントトルク$\tau_\chi$を実現する入力$\bm f_\text{r-}$をeq.~\eqref{eq:Mchi_quad}から求めることができる．
% \red{
% なお，eq.~\eqref{eq:M_quad}はランクが4であるため，一般には逆変換が存在しない．
% しかし，$^{b} f_{\text{rot}y}=0$である限り，$\chi$を調整することで逆変換が存在する}

\begin{remark}
    The control of the rigid body vehicle and the tilt angle of the quadlink are separable.

    From Eq.~\eqref{eq:Mchi_quad}, the thrust of the 5th and 6th rotors in $\bm f_\text{r-}$ can have arbitrary values. Therefore, a rotor thrusts $\bm f_\text{rot}$ corresponding to any $\bm f_\text{r+}$ and $\bm f_\text{r-}$ exists.
\end{remark}

\subsection{Aerodynamic Force}
In the previous subsection, we formulated the transformation of rotor thrusts. In cruise flight, aerodynamic forces also play a crucial role. In this subsection, we introduce aerodynamic forces.

The point of application of the aerodynamic force is assumed to be the same as the vehicle's center of gravity. Then, the aerodynamic force and torque are denoted as 
\begin{align}
    ^{s} \bm f_\text{aero} =& \begin{bmatrix}
                                  -D \\ 0 \\ -L
                              \end{bmatrix}, \label{eq:faero} \\
    ^{s} \bm \tau_\text{aero} =& \bm 0. \label{eq:tauaero}
\end{align}
Here, $L$ and $D$ represent the lift and drag forces, respectively. Their detailed expressions are provided as 
\begin{align}
    D =& \frac{1}{2} \rho ^{s}v_x^2 S C_D, \label{eq:D}\\
    L =& \frac{1}{2} \rho ^{s}v_x^2 S C_L. \label{eq:L}
\end{align}
where $\rho$ represents air density, $S$ is the wing area, and $C_L$ and $C_D$ are coefficients dependent on the angle of attack $\alpha$.
To determine $C_L$ and $C_D$, we approximate the results obtained from the work \cite{ozdemir_design_2014} using polynomial expressions.

% 空力のモデリングをする．
% 安定軸系での推力，モーメントは次のようにかける．
% \begin{align}
%     ^{s} \bm f_\text{aero} =& \begin{bmatrix}
%                                   -D \\ 0 \\ -L
%                               \end{bmatrix}, \label{eq:faero} \\
%     ^{s} \bm \tau_\text{aero} =& \bm 0. \label{eq:tauaero}                     
% \end{align}
% ここで，$L,~D$はそれぞれ揚力と抗力であり，次のように書ける．
% \begin{align}
%     D =& \frac{1}{2} \rho ^{s}v_x^2 S C_D, \label{eq:D}\\
%     L =& \frac{1}{2} \rho ^{s}v_x^2 S C_L. \label{eq:L}
% \end{align}
% ここで，$\rho$は空気密度，$S$は翼面積である．
% $C_D,~C_L$は迎角$\alpha$に依存する係数であり，解析では\cite{ozdemir_design_2014}の結果を多項式近似したものを用いる．

\subsection{Equation of Motion}
Let $\bm x\in\mbr^3$ represent the position of the vehicle in the inertial frame, $\bm v\in\mbr^3$ the velocity in the body frame, $\bm \eta \in\mbr^3$ the roll, pitch, and yaw angles, and $\bm \omega \in\mbr^3$ the angular velocity in the body frame. 

Derived from Eq.~\eqref{eq:Mf_quad}, \eqref{eq:Mtau_quad}, \eqref{eq:faero}, and \eqref{eq:tauaero}, the total thrust and moment around the center of gravity of the vehicle can be expressed as follows.
\begin{align}
    ^{b} \bm f =& ^{b} \bm f_\text{rot} + \bm R_y(\alpha)^\top {}^{s}\bm f_\text{aero} + \bm R_\eta^\top (m\bm g), \label{eq:FB} \\
    ^{b} \bm \tau =& ^{b} \bm \tau_\text{rot} + \bm R_y(\alpha)^\top {}^{s} \bm \tau_\text{aero}. \label{eq:MB}
\end{align}
, where $\bm g=[0~ 0~ g]^\top$ is the gravitational acceleration, and $\bm R_\eta$ is the rotation matrix due to the roll, pitch, and yaw angles.

The equation of motion for the aircraft can be expressed as follows.
\begin{align}
    & \dot{\bm x} = \bm R_\eta {}^{b}\bm v, \label{eq:navigation}\\
    & \dot{\bm\eta} = \begin{bmatrix}
        1 & \sin(\phi)\tan(\theta) & \cos(\phi)tan(\theta) \\
        0 & \cos(\phi) & -\sin(\phi) \\
        0 & \sin(\phi)/\cos(\theta) & \cos(\phi)/\cos(\theta)
    \end{bmatrix} {}^{b}\bm \omega, \label{eq:kinematics}\\
    & m^{b}\dot{\bm v} = -^{b}\bm\omega\times (m^{b}\bm v) + ^{b}\bm f, \label{eq:force}\\
    & \bm J^{b}\dot{\bm \omega} = -^{b}\bm\omega\times \bm J ^{b}\bm \omega + ^{b}\bm \tau  \label{eq:moment}.
\end{align}

% 状態$\bm x\in\mbr^3$を慣性座標における機体の位置，$\bm v\in\mbr^3$を機体速度，
% $\bm \eta \in\mbr^3$をロールピッチヨー角，$\bm \omega \in\mbr^3$を機体角速度とする．
% 機体の重心周りに働く推力・モーメントの合計は，eq.~\eqref{eq:Mf_quad}, eq.~\eqref{eq:Mtau_quad}, eq.~\eqref{eq:faero}, eq.~\eqref{eq:tauaero}から次のようにかける．
% \begin{align}
%     ^{b} \bm f =& ^{b} \bm f_\text{rot} + \bm R_y(\alpha)^\top {}^{s}\bm f_\text{aero} + \bm R_\eta^\top (m\bm g), \label{eq:FB} \\
%     ^{b} \bm \tau =& ^{b} \bm \tau_\text{rot} + \bm R_y(\alpha)^\top {}^{s} \bm \tau_\text{aero}. \label{eq:MB}
% \end{align}
% ここで，$\bm g=[0~ 0~ g]^\top$は重力加速度，$\bm R_\eta$は機体のロール・ピッチ・ヨー角$\eta$による回転行列である．

% 機体の運動方程式は次式のように表せる．
% \begin{align}
%     & \dot{\bm x} = \bm R_\eta {}^{b}\bm v, \label{eq:navigation}\\
%     & \dot{\bm\eta} = \begin{bmatrix}
%         1 & \sin(\phi)\tan(\theta) & \cos(\phi)tan(\theta) \\
%         0 & \cos(\phi) & -\sin(\phi) \\
%         0 & \sin(\phi)/\cos(\theta) & \cos(\phi)/\cos(\theta)
%     \end{bmatrix} {}^{b}\bm \omega, \label{eq:kinematics}\\
%     & m^{b}\dot{\bm v} = -^{b}\bm\omega\times (m^{b}\bm v) + ^{b}\bm f, \label{eq:force}\\
%     & \bm J^{b}\dot{\bm \omega} = -^{b}\bm\omega\times \bm J ^{b}\bm \omega + ^{b}\bm \tau  \label{eq:moment}.
% \end{align}


% ここで，$(\cdot)^\wedge$は歪対象行列を作る演算子である．
% なお，eq.\ref{eq:navigation}-\ref{eq:moment}は機体座標系での表現である．
% ここから平衡点入力の存在条件を議論するため，安定軸系での表現に書き換える．

% なお，ここでは平衡点は下記の条件を満たす状態のことをいう．
% \begin{itemize}
%     \item 安定軸系のx方向速度が一定$^{s}\bm v_x=\text{const.}$
%     \item その他の速度，及び角速度が$0$
% \end{itemize}
% また，安定軸系の$z$軸は重力方向と一致し，慣性座標の$x-y$平面と安定軸系の$x-y$平面は平行である．
% すなわち，$\phi=0,~\theta=\alpha,~\psi=0$であると仮定する．

% \end{document}


==> text/3-controllability.tex <==
% \documentclass[ieeeconf]{subfiles}
% \begin{document}

\section{STATIC HOVERING AND CRUISE REALIZABILITY}

\subsection{Realizability analysis of the vehicle}
In this subsection, we examine the feasibility of cruise flights. We start by defining cruise flight and then clarify the conditions necessary for achieving it, which are closely related to the hoverability of multicopters. Subsequently, a detailed analysis of these conditions is conducted.

\begin{definition}[Cruise flight]
    ${}^{s}v_x$をクルーズ速度とすると，機体が次の状態であるとき機体はクルーズ状態であるとする
    \begin{align*}
        \dot{\bm x}=[{}^{s}v_x~0~0]^\top,~^{s}\dot{\bm v}=\bm 0,~\dot{\bm\eta} = \bm 0,~\dot{\bm\omega} =\bm 0
    \end{align*}
\end{definition}
Additionally, we assume that the velocity during cruise flight is directed horizontally, namely the vehicle flight at a constant altitude in the inertial frame. In this case, the $x$-$y$ plane in the inertial frame is parallel with the $x$-$y$ plane in the stability frame, resulting in a complete alignment between the angle of attack $\alpha$ and the pitch angle $\theta$.
この仮定のもとでは，平衡点は以下のようになる．
\begin{align}
    {}^{b}\bm v =& \begin{bmatrix}
        {}^{s}v_x\cos{\alpha} & 0 & {}^{s}v_x\sin{\alpha}
    \end{bmatrix}^\top,\\
    \bm\eta =& \begin{bmatrix}
        0 & \alpha & 0
    \end{bmatrix},\\
    \bm \omega =& \begin{bmatrix}
        0 & 0 & 0
    \end{bmatrix}.\label{eq:equilibrium}
\end{align}
% \red{上の１つ目の式，色々と間違っていませんか？}
% なお，${}^{s}v_x=0$のときがHoveringである．さらに，本論文では簡単のためクルーズ飛行は慣性座標系で水平に飛行している状態とする．すなわち，高度が一定で飛行しており，安定軸系と慣性座標のx-y平面が平衡であることを示している．このとき，迎角$\alpha$とピッチ角$\theta$は完全に一致する．

As a preparation for the cruise flight condition, we introduce the hoverability condition of multicopters proven in \cite{9393789}.
% クルーズ飛行のrealizabilityを考えるために，まずはmulticopterのhoveringのrealizabilityを考える．
\begin{lemma}[Hoverability of the multicopter\cite{9393789}]\label{lem:hoverability}
    A multirotor UAV is hoverable if and only if the following two conditions are satisfied.
    \begin{enumerate}
        \item There exists input vector $\bm f_{r+}$ satisfying
            \begin{align*}
                \bm M \bm f_{r+} = \begin{bmatrix} -m\bm g\\ \bm O_{3\times 1} \end{bmatrix}. 
            \end{align*}
        \item The control effectiveness matrix $\bm M$ satisfies
            \begin{align*} \mathrm{rank}(\bm M) = 4. \end{align*}
    \end{enumerate}
\end{lemma}
The first condition in Lemma \ref{lem:hoverability} indicates the existence of the equilibrium input, and the second condition certifies the local controllability around the equilibrium point.
% この補題は，(1)が平衡点入力の存在条件を示しており，(2)が局所可制御性を保証している．
On the other hand, in the cruise flight, when viewed from a coordinate frame that moves in constant velocity with the vehicle, we can consider the vehicle as if it were hovering within the potential field made by gravity and the aerodynamic force. Therefore, by simply adjusting the equilibrium input, we can use almost the same satisfaction as follows.
% クルーズ状態についても，機体とともに定速で移動する座標系を考えたときに座標系の運動による慣性力等は発生しないため，重力と空力に釣り合う平衡点入力が存在すれば同様の条件を，
% クルーズ状態に対するrealizabilityの条件である下記を得る．
\begin{lemma}[Realizability of the cruise flight]\label{lem:cruisability}
    A vehicle achieves a cruise flight if and only if the following two conditions are satisfied.
    \begin{enumerate}
        \item \label{cruise_cond1}
            There exists input vector $\bm f_{r+}$ satisfying
            \begin{align} 
                \bm M \bm f_{r+} = 
                \begin{bmatrix} 
                    -\bm R_y(\alpha)^\top(^{s}\bm f_\text{aero} + m\bm g)\\
                    \bm O_{3\times 1} 
                \end{bmatrix}.\label{eq:cond1}
            \end{align}
        \item \label{cruise_cond2}
        The control effectiveness matrix $\bm M$ satisfies
            \begin{align*} \mathrm{rank}(\bm M) = 4. \end{align*}
    \end{enumerate}
\end{lemma}

提案機体について，このlemmaを満たす条件を次のTheremに示す．

% \red{The below subsections describe detailed analyses of these two conditions.
\begin{theorem}
    The proposed vehicle realizes a cruise flight when below conditions are satisfied. 
    \begin{enumerate}
        \item ${}^{s}v_x$, $\alpha$, and $\chi$ are in \red{a certain equilibrium state set, which is revealed below.}
        \item $\chi \in [-\pi/2,~0]$
    \end{enumerate}
\end{theorem}

\begin{proof}
    このtheremの二つの条件は，Lemma~\ref{lem:cruisability}の二つの条件からそれぞれ導くことができる．以下ではそれぞれの条件を順に証明していく．
    
    まず，Lemma~\ref{lem:cruisability}-\ref{cruise_cond1})から，Eq.~\eqref{eq:cond1}を安定軸径での表現に書き換えて移項すると．
    \begin{align}
        \begin{bmatrix}
            \bm R_y(\alpha) & \bm O_3 \\
            \bm O_3         & \bm I_3
        \end{bmatrix}\bm M \bm f_{r+} + 
        \begin{bmatrix}
            \bm (^{s}\bm f_\text{aero} + m\bm g)\\
            \bm O_{3\times 1} 
        \end{bmatrix}
        = \bm 0.
    \end{align}
    平衡点\eqref{eq:equilibrium}を代入し，対称の位置にあるロータに同じ推力，すなわち$f_1=f_3,~f_2=f_4,~f_5=f_6$を代入すると，
    % さらに，もともとy軸方向の推力は生成しないことから，平衡点入力は次の3式を満たせばよいことになる．
    \begin{align}
        \begin{bmatrix}
            -D - f_f\sin(\alpha+\chi) - f_b\sin(\alpha) \\
            0 \\
            mg - L - f_f\cos(\alpha+\chi) - f_b\cos(\alpha) \\
            0 \\
            f_f l_f \cos(\chi) - f_b l_b \cos(\chi) = 0 \\
            0 
        \end{bmatrix} = 
        \begin{bmatrix}
            0 \\ 0 \\ 0 \\ 0 \\ 0 \\ 0
        \end{bmatrix}
    \end{align}
    となる．これはx方向の力，z方向の力，y軸回りのモーメントが釣り合っている状態を表している．
    \red{fig.\ref{fig:sideview_force}を参照する．}
    \begin{figure}[t]
        % \begin{minipage}{0.48\linewidth}
            \centering
            \includegraphics[width=\linewidth]{"figure/controllability/sideview_force.eps"}
            \caption{平衡状態の推力}
            \label{fig:sideview_force}
        % \end{minipage}\hspace{2em}
    \end{figure}
    整理すると，次式が出てくる．
    \begin{align}
        (mg-L) \left(S_{\alpha+\chi}+\frac{l_f}{l_b}C_\chi S_\alpha\right)
        + D \left(C_{\alpha+\chi}+\frac{l_f}{l_b}C_\chi C_\alpha\right) = 0. \label{eq:alphachi_cond}
    \end{align}
    Eq.~\eqref{eq:alphachi_cond}を満たす$^{s}v_x\alpha,~\chi$の集合は，Fig.~\ref{fig:equilibrium}に示すような平面集合になる．
    このとき，機体には平衡点入力が存在し，Lemma~\ref{lem:cruisability}(\ref{cruise_cond1})を満たす．
    \begin{figure}[t]
        % \begin{minipage}{0.48\linewidth}
            \centering
            \includegraphics[width=\linewidth]{"figure/controllability/equilibrium.eps"}
            \caption{平行点入力が存在する$\alpha,~\chi$のマップ．}
            \label{fig:equilibrium}
        % \end{minipage}\hspace{2em}
    \end{figure}

    次にLemma~\ref{lem:cruisability}(\ref{cruise_cond2})を満たす条件を考える．
    Eq.~\eqref{eq:M}を
    \begin{align}
        \bm M 
        =& \left[\begin{array}{cc|cc}
            - S_\chi & - S_\chi & 0 & 0 \\
            0 & 0 & 0 & 0 \\
            \hline
            - C_\chi & - C_\chi & -1 & -1 \\
            -l_{fw} C_\chi-\kappa S_\chi &l_{fw} C_\chi+\kappa S_\chi & -l_{bw} & l_{bw} \\
            \hline
            l_{f} C_\chi & l_{f} C_\chi & -l_b & -l_b \\
            l_{fw} S_\chi-\kappa C_\chi & -l_{fw} S_\chi+\kappa C_\chi & \kappa & -\kappa
        \end{array}\right] \notag\\
        = & 
        \left[\begin{array}{c|c}
            \bm M_{11} & \bm M_{12} \\
            \hline
            \bm M_{21} & \bm M_{22} \\
            \hline
            \bm M_{31} & \bm M_{32}
        \end{array}\right].
    \end{align}
    のように分割すると，
    \begin{align}
        \mathrm{rank}(\bm M)&=
        \mathrm{rank}(\bm M_{22}) + \mathrm{rank}(\bm M_{31})
    \end{align}
    となり，自明に$\mathrm{rank}(\bm M_{22})=2$である．
    また，$\chi=[-\pi/2,~0]$のとき$\mathrm{rank}(\bm M_{31})=2$となり，$\mathrm{rank}(\bm M)=4$となる．
    
    以上でLemma~\ref{lem:cruisability}の二つの条件を満たす$\alpha,~\chi,~{}^{s}v_x$についての条件を導出できた．
\end{proof}

% \subsection{平衡点入力の存在条件}
% 機体座標系と安定軸系間の回転$\bm R_y(\alpha)$を用いて
% eq.\ref{eq:navigation}-\ref{eq:moment}を書き換え，整理すると．
% \begin{align}
%     & \dot{\bm x} = \bm R(\eta) \bm R_y^\top(\alpha) {}^{s}\bm v, \label{eq:navigation_s}\\
%     & \dot{\bm\eta} = \begin{bmatrix}
%         1 & \sin(\phi)\tan(\theta) & \cos(\phi)tan(\theta) \\
%         0 & \cos(\phi) & -\sin(\phi) \\
%         0 & \sin(\phi)/\cos(\theta) & \cos(\phi)/\cos(\theta)
%     \end{bmatrix} \bm R_y^\top(\alpha) {}^{s}\bm \omega, \label{eq:kinematics_s}\\
%     & m^{s}\dot{\bm v} = -^{s}\bm\omega\times (m^{s}\bm v) + ^{s}\bm f, \label{eq:force_s}\\
%     & \tilde{\bm J}^{s}\dot{\bm \omega} = -^{s}\bm\omega\times \tilde{\bm J} ^{s}\bm \omega + ^{s}\bm \tau  \label{eq:moment_s}.
% \end{align}
% となる．ここで，$\tilde{\bm J}=\bm R_y(\alpha)\bm J \bm R_y^\top(\alpha)$である．
% これらに平衡点$^{s}\bm v=[^{s}v_x~0~0]^\top,~^{s}\bm\omega=\bm 0,~\eta=[0~\alpha~0]^\top$を代入すると，eq.\eqref{eq:navigation}, eq.\eqref{eq:kinematics}は恒等式になり，
% eq.\eqref{eq:force},~eq.\eqref{eq:moment}は次のようになる．
% \begin{align}
%     ^{s}\bm f = \bm 0 \\
%     ^{s}\bm \tau = \bm 0
% \end{align}

% \subsection{可制御性}
% \begin{theorem}[Realizability]
%     Eq.~\eqref{eq:alphachi_cond}を満たし，かつ$\chi=[-\pi/2,~0]$のとき，機体はクルーズ飛行可能である．
% \end{theorem}
% \begin{proof}

% \end{proof}

\subsection{Planning of $\alpha$ and $\chi$}

\begin{figure}[t]
    % \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{"figure/controllability/equilibrium_topview.eps"}
        \caption{平行点入力が存在する$\alpha,~\chi$のマップ．}
        \label{fig:equilibrium_topview}
    % \end{minipage}\hspace{2em}
\end{figure}
    
上記の結果を用いて機体のtransition時の迎角$\alpha$，チルト角$\chi$を計画する．
Fig.~\ref{fig:equilibrium}の平面上にあるときにcruise flight可能であり，この平面上でtransitionの時系列変化をプランニングする．
この平面上で目的関数等を設定して最適パスを計画することも考えられるが，本論文の主旨は機体の提案とクルーズ可能条件の証明，シミュレーションによる決定のみであるため，最適設計は今後の課題とする．

本シミュレーションでは，$\alpha$と$\chi$平面への射影が線形に変化するパスを考える．
\red{詳しく説明or Fig5の上から見た図を添付（後者がわかりやすいかな）}

なお，これは平衡点に限った入力であり，動的に制御するにはこの値では不十分である．いずれかの変数を使って制御する必要がある．
${}^{s}v_x,~\alpha$はEq.~\eqref{eq:D},~\eqref{eq:L}に示す通り空力に非線形に関係する変数であり，値を変化させると空力が変化してダイナミクスが複雑になってしまう．そのため，シミュレーションでは$\chi$を変化させて制御する．詳細な説明はcontrollerの章にしめす．


% \end{document}
